On the geometry of the set of symmetric matrices with repeated eigenvalues

We investigate some geometric properties of the real algebraic variety $\Delta$ of symmetric matrices with repeated eigenvalues. We explicitly compute the volume of its intersection with the sphere and prove a Eckart-Young-Mirsky-type theorem for the distance function from a generic matrix to points in $\Delta$. We exhibit connections of our study to Real Algebraic Geometry (computing the Euclidean Distance Degree of $\Delta$) and Random Matrix Theory.

==> header.tex <==
% PACKAGES
\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage[babel]{csquotes}
\usepackage{tikz}
\usepackage{amsthm}
\usepackage{amsmath,amssymb}
\usepackage[title,titletoc]{appendix}
%\usepackage{mathtools}
%\mathtoolsset{showonlyrefs=false}
%\usepackage[format=plain, font=footnotesize]{caption}
\usepackage[colorlinks=true, citecolor=\citecolor, linkcolor=\linkcolor]{hyperref}
\usepackage[english]{cleveref}
\usepackage{color,calc,comment}
\usepackage{enumitem}
\usepackage{bbm}
\usepackage{euscript}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{tkz-euclide, tikz}
\usetikzlibrary{backgrounds,patterns,matrix,calc,arrows,positioning,fit,shapes.geometric,decorations.pathmorphing}
\pgfdeclarelayer{bg}
\pgfdeclarelayer{bg2}    % declare background layer
\pgfsetlayers{bg2,bg,main}
\usepackage{wrapfig}
\setenumerate{labelsep=*, leftmargin=1.5pc}
%\setenumerate[1]{label=\arabic*., ref=\arabic*}

%DEFINITIONS
\newcommand{\HA}{\mathbb{A}}
\newcommand{\HB}{\mathbb{B}}
\newcommand{\HC}{\mathbb{C}}
\newcommand{\HD}{\mathbb{D}}
\newcommand{\HE}{\mathbb{E}}
\newcommand{\HF}{\mathbb{F}}
\newcommand{\HG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\HI}{\mathbb{I}}
\newcommand{\HJ}{\mathbb{J}}
\newcommand{\HK}{\mathbb{K}}
\newcommand{\HL}{\mathbb{L}}
\newcommand{\HM}{\mathbb{M}}
\newcommand{\HN}{\mathbb{N}}
\newcommand{\HO}{\mathbb{O}}
\newcommand{\HP}{\mathbb{P}}
\newcommand{\HQ}{\mathbb{Q}}
\newcommand{\HR}{\mathbb{R}}
\newcommand{\HS}{\mathbb{S}}
\newcommand{\HT}{\mathbb{T}}
\newcommand{\HU}{\mathbb{U}}
\newcommand{\HV}{\mathbb{V}}
\newcommand{\HW}{\mathbb{W}}
\newcommand{\HX}{\mathbb{X}}
\newcommand{\HY}{\mathbb{Y}}
\newcommand{\HZ}{\mathbb{Z}}

\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sE}{\mathscr{E}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sI}{\mathscr{I}}
\newcommand{\sJ}{\mathscr{J}}
\newcommand{\sK}{\mathscr{K}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sO}{\mathscr{O}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sQ}{\mathscr{Q}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\sS}{\mathscr{S}}
\newcommand{\sT}{\mathscr{T}}
\newcommand{\sU}{\mathscr{U}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sW}{\mathscr{W}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}


\newcommand{\bQ}{\underline{Q}}
\newcommand{\bM}{\mathbf{M}}


\newcommand{\ka}{\mathfrak{a}}
\newcommand{\kb}{\mathfrak{b}}
\newcommand{\kc}{\mathfrak{c}}
\newcommand{\kd}{\mathfrak{d}}
\newcommand{\ke}{\mathfrak{e}}
\newcommand{\kf}{\mathfrak{f}}
\newcommand{\kg}{\mathfrak{g}}
\newcommand{\kh}{\mathfrak{h}}
\newcommand{\ki}{\mathfrak{i}}
\newcommand{\kj}{\mathfrak{j}}
\newcommand{\kk}{\mathfrak{k}}
\newcommand{\kl}{\mathfrak{l}}
\newcommand{\km}{\mathfrak{m}}
\newcommand{\kn}{\mathfrak{n}}
\newcommand{\ko}{\mathfrak{o}}
\newcommand{\kp}{\mathfrak{p}}
\newcommand{\kq}{\mathfrak{q}}
\newcommand{\kr}{\mathfrak{r}}
\newcommand{\ks}{\mathfrak{s}}
\newcommand{\kt}{\mathfrak{t}}
\newcommand{\ku}{\mathfrak{u}}
\newcommand{\kv}{\mathfrak{v}}
\newcommand{\kw}{\mathfrak{w}}
\newcommand{\kx}{\mathfrak{x}}
\newcommand{\ky}{\mathfrak{y}}
\newcommand{\kz}{\mathfrak{z}}
\newcommand{\kA}{\mathfrak{A}}
\newcommand{\kB}{\mathfrak{B}}
\newcommand{\kC}{\mathfrak{C}}
\newcommand{\kD}{\mathfrak{D}}
\newcommand{\kE}{\mathfrak{E}}
\newcommand{\kF}{\mathfrak{F}}
\newcommand{\kG}{\mathfrak{G}}
\newcommand{\kH}{\mathfrak{H}}
\newcommand{\kI}{\mathfrak{I}}
\newcommand{\kJ}{\mathfrak{J}}
\newcommand{\kK}{\mathfrak{K}}
\newcommand{\kL}{\mathfrak{L}}
\newcommand{\kM}{\mathfrak{M}}
\newcommand{\kN}{\mathfrak{N}}
\newcommand{\kO}{\mathfrak{O}}
\newcommand{\kP}{\mathfrak{P}}
\newcommand{\kQ}{\mathcal{Q}}
\newcommand{\kR}{\mathfrak{R}}
\newcommand{\kS}{\mathfrak{S}}
\newcommand{\kT}{\mathfrak{T}}
\newcommand{\kU}{\mathfrak{U}}
\newcommand{\kV}{\mathfrak{V}}
\newcommand{\kW}{\mathfrak{W}}
\newcommand{\kX}{\mathfrak{X}}
\newcommand{\kY}{\mathfrak{Y}}
\newcommand{\kZ}{\mathfrak{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand\restr[2]{\ensuremath{\left.#1\right|_{#2}}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\cset}[2]{\left\{#1\mid #2\right\}}
\newcommand{\rank}{\mathrm{rk}\,}
\newcommand{\id}{\mathrm{id}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\tlambda}{\tilde{\lambda}}
\newcommand{\tlambdamin}{\tlambda_{\min}}
\newcommand{\lambdamin}{\lambda_{\min}}
\newcommand{\tmu}{\tilde{\mu}}
\renewcommand{\d}{\mathrm{ d}}
\renewcommand{\dot}[1]{\overset{\raisebox{-0.25ex}{\scalebox{0.4}{$\bullet$}}}{#1}}
\newcommand{\Tang}[2]{\mathrm{T}_{#1}#2}
\DeclareMathOperator*{\Prob}{\mathrm{Prob}}
\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
\DeclareMathOperator*{\mean}{\mathbb{E}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

% COUNTER/LAYOUT CONFIGURATION
\numberwithin{equation}{section}
\numberwithin{figure}{section}
%THEOREMS
\theoremstyle{plain}
\newcounter{numbering} \numberwithin{numbering}{section}
\newtheorem{thm}[numbering]{Theorem}
\newtheorem{lemma}[numbering]{Lemma}
\newtheorem{prop}[numbering]{Proposition}
\newtheorem{cor}[numbering]{Corollary}
\theoremstyle{definition}
\newtheorem{dfn}[numbering]{Definition}
\newtheorem{notation}[numbering]{Notation}
\theoremstyle{remark}
\newtheorem*{claim}{Claim}

\newtheorem*{rem}{Remark}
\newtheorem{example}{Example}
% CLEVEREF
\crefname{equation}{}{}
\crefname{equation}{}{}
\crefname{figure}{Figure}{Figures}
\crefname{section}{Section}{Sections}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{prop}{Proposition}{Propositions}
\crefname{thm}{Theorem}{Theorems}
\crefname{cor}{Corollary}{Corollaries}
\crefname{dfn}{Definition}{Definitions}
\crefname{notation}{Notations}{Notations}
\crefname{rem}{Remark}{Remarks}
\crefname{claim}{Claim}{claims}
\pagestyle{plain}
\parindent0.5cm

